Causally consistent dynamic slicing

We offer a lattice-theoretic account of dynamic slicing for {\pi}-calculus, building on prior work in the sequential setting. For any run of a concurrent program, we exhibit a Galois connection relating forward slices of the start configuration to backward slices of the end configuration. We prove that, up to lattice isomorphism, the same Galois connection arises for any causally equivalent execution, allowing an efficient concurrent implementation of slicing via a standard interleaving semantics. Our approach has been formalised in the dependently-typed language Agda.

==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012, 2013, 2014, 2015: Matthieu Moy <Matthieu.Moy@imag.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use Pod::Usage;
use IO::Handle;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
if (!$TEXINPUTS) { $TEXINPUTS = getcwd(); }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $fatal;
my $version;
my $makeatletter;

GetOptions (
	'h' => \$help,
	'help' => \$long_help,
	'verbose|v' => \$verbose,
	'keep-comments' => \$keep_comments,
	'keep-includes' => \$keep_includes,
	'empty-comments' => \$empty_comments,
	'output|o=s' => \$output,
	'explain' => \$explain,
	'show-graphics' => \$show_graphics,
	'graphics-extensions' => \$graphics_extensions,
	'expand-usepackage' => \$expand_usepackage,
	'expand-bbl=s' => \$expand_bbl,
	'fatal' => \$fatal,
	'version' => \$version,
        'makeatletter' => \$makeatletter,
) or pod2usage(2);
version() if $version;
pod2usage(1) if $help;
pod2usage(-exitstatus => 0, -verbose => 2) if $long_help;

sub get_version
{
	# $VERSION's value will be substituted by 'make dist', but the
	# next line won't (the string has to be broken to avoid it).
	my $VERSION = 'v1.2-1-g47e2cee';
	if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
		my($vol,$dir,$file) = File::Spec->splitpath($0);
		chdir($dir);
		$VERSION = `git describe --tags HEAD 2>/dev/null`;
	}
	if ($VERSION eq '') {
		$VERSION = '<unknown version>';
	}
	$VERSION =~ s/^\s+|\s+$//g;
	return $VERSION;
}

sub version
{
	print "latexpand version ". get_version() .".\n";
	exit(0);
}

my $nl = "";
if ($empty_comments) {
	$nl = "%\n";
}

if ($output && $output ne "-") {
	open OUTPUT, '>', "$output" or die $!;
	STDOUT->fdopen(\*OUTPUT, 'w') or die $!;
}

sub say
{
	if ($verbose) {
		print STDERR "$_[0]";
	}
}

my $makeatletter_found;
my $in_preamble;

foreach my $file (@ARGV)
{
	say "processing $file\n";
	$makeatletter_found = 0;
	$in_preamble = 1;
	process_file($file, "  ");
}

sub process_file
{
	my $file = shift;
	my $prefix = (shift || "");
	my $in_comment = 0;
	local(*FILE);
	open(FILE, $file) or die "could not open input file '$file'\n";
	while (my $line = <FILE>) {
		if ($line =~ /^[ \t]*\\endinput/) {
			$line =~ s/(\\endinput.*)\n/% $1/;
			$in_comment = 1;
			process_line($line, $prefix);
			last;
		}
		process_line($line, $prefix, $file);
		if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
			# file ends with a comment not ending with a newline
			print "\n";
		}
		# Garbage at end of line after \end{document} is
		# ignored by LaTeX, but we don't allow anything before
		# to avoid e.g. \verb|\end{document}| from terminating
		# the file.
		if (!$keep_comments && $line =~ /^[ \t]*\\end{document}/) {
			last;
		}
	}
	close(FILE);
	return $in_comment;
}

sub process_line
{
	my ($_, $prefix, $file) = @_;
	# Consider \makeatletter only in preamble, because we do want
	# to warn on \someCommand{\makeatletter\command@with@arobase}.
	if ($in_preamble && /^[^%]*\\makeatletter/) {
		$makeatletter_found = 1;
	}
	if ($in_preamble && /^[^%]*\\makeatother/) {
		$makeatletter_found = 0;
	}
	if (!$makeatletter && !$makeatletter_found
	    && (my ($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)) {
		print STDERR "Warning: command $command containing @ found in\n";
		print STDERR "Warning: $file.\n";
		print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
	}
	unless ($keep_comments) {
		if ($empty_comments) {
			s/^%.*$/%/;
			s/([^\\])%.*$/$1%/;
		} else {
			s/^%.*\n//;
			s/([^\\])%.*\n/$1/;
		}
	}

	unless ($keep_includes) {
		if (my ($before, $ignored, $full_filename, $after)
		    = /^(([^%]|[^\\]%)*)\\include[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename . ".tex");
			if ($full_filename) {
				say $prefix . "Found include for file: $full_filename\n";
				print $before . $nl;
				print '\clearpage{}' . $nl;
				print "% start include $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end include $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				print '\clearpage{}' . $nl;
				print $nl . $after . "\n";
				$_ = "";
			}
		} elsif (my ($before, $ignored, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\input[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		}
	}
	if ($expand_usepackage) {
		# Don't bother with before and after text, we just require the
		# usepackage to be alone on its line.
		if (my ($package_name) = /^\s*\\usepackage{([^}]*)}\s*(%.*)?$/) {
			my $full = find_file($package_name . ".sty", $TEXINPUTS);
			if ($full) {
				say $prefix . "Found package file: $full\n";
				process_file($full, $prefix . "  ");
				$_ = "";
			} else {
				say $prefix . "Not including external package $package_name\n";
			}
		}
	}
	if ($expand_bbl) {
		if (my ($before, $bib_name, $after)
			 = /^(.*)\\bibliography{([^}]*)}(.*)$/) {
			# The BBL file is not necessarily $bib_name.
			# Take it from the command-line.
			print $before . $nl;
			say $prefix . "Expanding BBL file: $expand_bbl\n";
			process_file($expand_bbl, $prefix . "  ");
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($show_graphics) {
		if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
			my $full = find_tex_file($2, $graphics_extensions);
			say $prefix . "needs graphics file: ";
			print STDERR "$full\n";
		}
	}
	if (/^[ \t]*\\begin{document}/) {
		$in_preamble = 0;
		if ($makeatletter) {
			print '\makeatletter' . $nl;
		}
	}
	print;
}

# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
	my $file = shift;
	my $extensions = (shift || ":");
	foreach my $ext (split(':', $extensions, -1)) {
		my $full = find_file($file . $ext, $TEXINPUTS);
		if ($full) {
			return $full;
		}
	}
	if ($fatal) {
		die "ERROR: Could not find file [$file]\n";
	} else {
		print STDERR "Warning: Could not find file [$file]\n";
		return undef;
	}
}

sub find_file
{
	my ($file, $path) = @_;
	if (File::Spec->file_name_is_absolute($file)) {
		if (-e "$file" && ! -d "$file") {
			return $file;
		} else {
			return;
		}
	}
	foreach my $dir (split(':', $path)) {
		if (-e "$dir/$file" && ! -d "$dir/$file") {
			return("$dir/$file");
		}
	}
	return;
}


__END__

=head1 NAME

latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments

=head1 SYNOPSIS

latexpand [options] FILE...

=head2 Options:

	--verbose        show what's going on
	--keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
	--empty-comments keep empty comments (i.e. % at end of lines) for clarity
	--keep-includes  don't expand \input and \include directives
	--expand-usepackage
	                 Expand \usepackage{...} directives if the
	                 corresponding .sty file is found in
	                 $TEXINPUTS (or the current directory if
	                 $TEXINPUTS is not set)
	--expand-bbl FILE
	                 Expand the bibliography by inlining FILE
	                 (should be a *.bbl file)
	--help           this help message
	--output <file>, -o <file>
	                 generate output in <file>
	--explain        generate explanatory comments in output
	--show-graphics  show included graphics
	--graphics_extensions
	                 colon-separated list of possible graphics extensions
	                 (used by --show-graphics to find the actual graphics files)
	--fatal          Die in case a file can't be found.
	--makeatletter   Insert a \makeatletter in the preamble. In some
	                 rare cases it may break your document, but it
	                 may help fixing bad interactions between
	                 @-commands and inclusion (see BUGS section).

=head1 USES

The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.

=head1 GETTING LATEXPAND

The latest version of latexpand is available here:

  https://gitorious.org/latexpand

Versions are uploaded to ctan.org from time to time:

  http://www.ctan.org/pkg/latexpand

=head1 BUGS

Please, report bugs to Matthieu Moy <Matthieu.Moy@imag.fr>.

=head2 Known bugs

=head3 Verbatim

latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).

=head3 Comment environment

It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.

Code like

	foo%
	\begin{comment}

will produce the incorrect

	foo\begin{comment}

A workaround is to use --empty-comments when such tricky usage of the
comments package is done.

=head3 \makeatletter and use with transfig/xfig with \scalebox{}

If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.

This happens with

	\scalebox{ \input{file-generated-by-xfig.pdf_t} }

Workaround: add \makeatletter before the scalebox manually in your
code, like

        \makeatletter{}
	\scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}

In the case of xfig generated files, it is necessary only for the
first occurence.

A more brute-force workaround is to use latexpand --makeatletter.

=head1 SEE ALSO

Instructions to include only the relevant .bib items (french):

https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances

=head1 VERSION

This is latexpand version v1.2-1-g47e2cee.


==> notes.tex <==
Concurrency and slicing

Given a concurrent system, suppose it runs and reaches a final state with something ``wrong'' with it.  We would like to understand what went wrong and how the system reached that state.  More generally, we would like to have a way of understanding one (or comparing several) ``runs'' of the system.

The obvious notion of ``run'' is a sequence of system states, linked by (possibly labelled) transitions.  However, this seems unnecessarily low-level; it provides all of the information about the sequence of states but very little information about how they are related.  One must manually inspect two adjacent states, taking their label into account, to infer what action took place in the transition between the first state and the second.  Moreover, the sequence of states imposes an unnecessary linearization of the run, so that two causally-related steps might be separated by arbitrarily many unrelated steps.  A given run can have many causally equivalent linearizations, which means that comparing the linearizations of two runs of a system is not a good way to compare their actual behavior.

Another natural alternative is to construct a graph where nodes are events and edges are causal dependencies between events.  This approach has been explored extensively in informal settings, under the names provenance graph, causality graph, etc.  However, to our knowledge there is no prior work formally connecting such graphs with the behavior of a concurrency calculus.  Most such techniques have been developed in response to needs enunciated by scientific users of high-performance computation systems (e.g. scientific workflow systems) in order to make the computational process more transparent and aid in tracking down anomalies.  However, it is not clear whether such provenance graphs actually provide enough information to meet specific needs.

Consider the following concrete scenario: A scientist (possibly with the aid of other computing staff) develops a new analysis to run on genomic and proteomic data.  The computation requires running large subroutines on large amounts of data in ``chunks'',  and to improve performance the computation is distributed across a number of computers.  A relatively small amount of code is written to coordinate the behavior of the processes; the computation is not simply ``embarrassingly parallel'' but instead the coordination process adaptively decides on further subroutines to run depending on the results of earlier ones.  For example, the system might initially run a ``parameter sweep'' to compare the predictions of a model to some data, then depending on the results, focus on certain interesting regions of the parameter space.  In a real setting, this coordination code might be written in a programming or scripting language such as Java, Python, or R, using low-level communication primitives; however, here we will model the coordination of the processes using a process calculus.

Now suppose the computation runs, and a few days later some results are produced.  Some of them seem reasonable, but others are extremely strange.  If the system does not provide any tracing or provenance records that would aid the scientist in understanding the intermediate decisions made by the coordination, it is far from clear how a given output (or part of the output) is related to the source.  Anomalous results are worrying because they suggest that the plausible results might also be incorrect.  Even if all of the results appear correct, the scientist would probably like to pay extra attention to certain interesting results that might form the basis of a publication, to ensure that the computations leading to them were actually correct.  (Failure to do so has done major damage to some scientists’ careers.) 

Moreover, suppose the scientist runs the computation again on the same data, and obtains different results --- this is totally plausible because the concurrent coordination process is nondeterministic.  Again, the scientist is not going to be happy: the computational ``experiment'' is not even reproducible!  Similarly, the scientist could change the data or process slightly and rerun, but there is no guarantee that the resulting run will bear any resemblance to the original one, making it difficult to make sense of any differences observed in the results.
